Response to David Steigmann's discussion of our paper

We respond to David Steigmann's discussion of our paper "A general theory for anisotropic Kirchhoff-Love shells with in-plane bending of embedded fibers, Math. Mech. Solids, 28(5):1274-1317" (arXiv:2101.03122). His discussion allows us to clarify two misleading statements in our original paper, and confirm that its formulation is fully consistent with the formulation of Steigmann. We also demonstrate that some of our original statements criticized by Steigmann are not wrong.

==> neco_updated.tex <==


\makeatletter
\DeclareRobustCommand*\ouell{\mathpalette\@ouell\relax}
\newcommand*\@ouell[2]{
  % We need to adjust the width of \uell to be the same as \ell
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.4ex \hbox{\kern \dimen0\unhbox1\kern \dimen0}}
}

\makeatletter
\DeclareRobustCommand*\houell{\mathpalette\@houell\relax}
\newcommand*\@houell[2]{
  % We need to adjust the width of \uell to be the same as \ell
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.2ex \hbox{\kern \dimen0\unhbox1\kern \dimen0}}
}

\newcommand{\widerbar}[1]{\mskip.5\thinmuskip\overline{\mskip-1\thinmuskip {#1} \mskip-.5\thinmuskip}\mskip.5\thinmuskip} % overline short


%for Gamma^\uell
%\newcommand {\uell}{\scaleto{\boldsymbol{\ouell}\mathstrut}{6.5pt}}
\newcommand {\uell}{\scaleto{{\ouell}\mathstrut}{6.5pt}}


%for L^\huell
%\newcommand {\huell}{\scaleto{\boldsymbol{\houell}\mathstrut}{6.5pt}}
\newcommand {\huell}{\scaleto{{\houell}\mathstrut}{6.5pt}}


%moving hat left
\newcommand*{\xhat}[1]{#1\kern-0.75em\hat{\phantom{#1}}}

\newcommand {\Lhat}{\mathrm{\xhat{L}}}



% Equations
\newcommand{\bitm}{\begin{itemize}}
\newcommand{\eitm}{\end{itemize}}
\newcommand{\bnumr}{\begin{enumerate}}
\newcommand{\enumr}{\end{enumerate}}
\newcommand{\bolds}[1]{\boldsymbol{#1}}
\newcommand {\nqp}{n_\mathrm{qp}}
\newcommand {\ngp}{n_\mathrm{qp}}
\newcommand {\wqp}{w_\mathrm{qp}}
\newcommand {\wgp}{w_\mathrm{qp}}

\newcommand {\sigab}{\sigma^{\alpha\beta}}
\newcommand {\ellab}{\ell^{\alpha\beta}}

\newcommand {\divv}{\mathrm{div}}
\newcommand {\smallSigma}{\scaleto{\Sigma\mathstrut}{6pt}}
\newcommand {\smallLambda}{\scaleto{\Lambda\mathstrut}{6pt}}


\newcommand {\ella}{\ell^{\alpha}}
\newcommand {\ellb}{\ell^{\beta}}

\newcommand {\nbara}{\bar{n}^{\alpha}}
\newcommand {\nbarb}{\bar{n}^{\beta}}

\newcommand {\sigbar}{\bar{\sigma}}
\newcommand {\sigmabar}{\bar{\sigma}}
\newcommand {\taubar}{\bar{\tau}}
\newcommand {\sbar}{\bar{s}}

\newcommand {\aab}{a^{\alpha\beta}}
\newcommand {\auab}{a_{\alpha\beta}}
\newcommand {\agd}{a^{\gamma\delta}}
\newcommand {\abd}{a^{\beta\delta}}
\newcommand {\abg}{a^{\beta\gamma}}
\newcommand {\aad}{a^{\alpha\delta}}
\newcommand {\aag}{a^{\alpha\gamma}}

\newcommand {\augd}{a_{\gamma\delta}}
\newcommand {\augb}{a_{\gamma\beta}}
\newcommand {\aute}{a_{\theta\epsilon}}

\newcommand {\adb}{a^{\delta\beta}}
\newcommand {\aga}{a^{\gamma\alpha}}

\newcommand {\Aab}{A^{\alpha\beta}}
\newcommand {\Auab}{A_{\alpha\beta}}
\newcommand {\Agd}{A^{\gamma\delta}}
\newcommand {\Augd}{A_{\gamma\delta}}

\newcommand {\Mab}{M^{\alpha\beta}}
\newcommand {\mab}{m^{\alpha\beta}}
\newcommand {\Mbarab}{\bar{M}^{\alpha\beta}}

\newcommand {\Mhatab}{\hat{M}^{\alpha\beta}}

\newcommand {\Mhat}{\hat{M}}

\newcommand {\mbar}{\bar{m}}
\newcommand {\mhat}{\hat{m}}


\newcommand {\Nab}{N^{\alpha\beta}}
\newcommand {\Nbarab}{\bar{N}^{\alpha\beta}}


\newcommand {\Muab}{M_{\alpha\beta}}
\newcommand {\Mgd}{M^{\gamma\delta}}
\newcommand {\Mgb}{M^{\gamma\beta}}
\newcommand {\Mugd}{M_{\gamma\delta}}

\newcommand {\bab}{b^{\alpha\beta}}

\newcommand {\buab}{b_{\alpha\beta}}
\newcommand {\baug}{b^{\alpha}_{\gamma}}
\newcommand {\bgd}{b^{\gamma\delta}}
\newcommand {\bgb}{b^{\gamma\beta}}
\newcommand {\bugd}{b_{\gamma\delta}}
\newcommand {\tbgd}{\tilde{b}^{\gamma\delta}}
\newcommand {\tauab}{\tau^{\alpha\beta}}

\newcommand{\mcalC}{\mathcal{C}}
\newcommand{\mcalS}{\mathcal{S}}

\newcommand{\mrN}{\mathrm{N}}
\newcommand{\mrD}{\mathrm{D}}
\newcommand{\mrT}{\mathrm{T}}
\newcommand{\mrL}{\mathrm{L}}
\newcommand{\bnP}{\bn_\mathrm{p}}
\newcommand{\mrin}{\mathrm{in}}



\newcommand {\eqb}[1]{\begin{equation}\begin{array}{#1}}
\newcommand {\eqe}{\end{array}\end{equation}}
\newcommand {\eqbb}[1]{\begin{equation}\boxed{\begin{array}{#1}}
\newcommand {\eqeb}{\end{array}}\end{equation}}
\newcommand {\esb}[1]{\begin{equation*}\begin{array}{#1}}
\newcommand {\ese}{\end{array}\end{equation*}}
\newcommand {\ds}{\displaystyle}
\newcommand {\ts}{\textstyle}
\newcommand {\df}[2]{\frac{\ds#1}{\ds#2}}
\newcommand {\pa}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand {\paq}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}}
\newcommand {\pad}[2]{\frac{\mathrm{d}{#1}}{\mathrm{d}{#2}}}
\newcommand {\paqq}[3]{\frac{\partial^2{#1}}{\partial{#2}\,\partial{#3}}}
\newcommand {\back}{\! \! \!}
\newcommand {\is}{\back &=& \back}
\newcommand {\dis}{\back &:=& \back}
\newcommand {\isd}{\back &=:& \back}
\newcommand {\ais}{\back &\approx& \back}
\newcommand {\isn}{\back &\neq& \back}
\newcommand {\plus}{\back &+& \back}
\newcommand {\mi}{\back &-& \back}
\newcommand {\isl}{\back &<& \back}
\newcommand {\isleq}{\back &\leq& \back}
\newcommand {\isg}{\back &>& \back}
\newcommand {\isgeq}{\back &\geq& \back}
\newcommand {\isin}{\back &\in& \back}
\newcommand {\with}{\quad,$with:$\quad}
\newcommand {\s}{~\!}

% Functions
\newcommand {\mc}[3]{\multicolumn{#1}{#2}{#3}}
\newcommand {\norm}[1]{\|#1\|}
\newcommand {\tr}{\mathrm{tr}\,}
\newcommand {\sign}{\mathrm{sign}\,}
\newcommand {\spur}{\mathrm{sp}\,}
\newcommand {\grad}{\mathrm{grad}\,}
\newcommand {\divz}{\mathrm{div}\,}
\newcommand {\rot}{\mathrm{rot}\,}
\newcommand {\Grad}{\mathrm{Grad}\,}
\newcommand {\Divz}{\mathrm{Div}\,}

% Differential
\newcommand {\dif}{\mathrm{d}}

% Average
\newcommand {\ave}[1]{\langle#1\rangle}
\newcommand {\avo}[1]{\langle #1 \rangle_{\Omega}}
\newcommand {\ava}[1]{\langle #1 \rangle_{\Omega_e}}
\newcommand {\avb}[1]{\langle #1 \rangle_{\Omega/\Omega_e}}
\newcommand {\avI}[1]{\langle #1 \rangle_{\Omega_I}}
\newcommand {\avE}[1]{\langle #1 \rangle_{\Omega_E}}
\newcommand {\iom}{\int_\Omega}
\newcommand {\pom}{\int_{\partial\Omega}}

% Invariants
\newcommand {\II}{{I\kern-.3em I}}
\newcommand {\III}{{I\kern-.3em I\kern-.3em I}}

% Integrals
\newcommand {\into}{\int_\Omega}
\newcommand {\intoo}{\int_{\Omega_0}}
\newcommand {\intI}{\int_{\Omega_I}}
\newcommand {\inta}{\int_{\Omega_1}}
\newcommand {\intb}{\int_{\Omega_2}}
\newcommand {\intc}{\int_{\Omega_3}}
\newcommand {\inti}{\int_{\Omega_i}}
\newcommand {\intj}{\int_{\Omega_j}}
\newcommand {\intk}{\int_{\Omega_k}}
\newcommand {\intl}{\int_{\Omega_\ell}}
\newcommand {\intab}{\int_{\bar{\Omega}_1}}
\newcommand {\intbb}{\int_{\bar{\Omega}_2}}
\newcommand {\intcb}{\int_{\bar{\Omega}_3}}
\newcommand {\intaob}{\int_{\bar{\Omega}_{10}}}
\newcommand {\intbob}{\int_{\bar{\Omega}_{20}}}
\newcommand {\intaobb}{\int_{\bar{\bar{\Omega}}_{10}}}
\newcommand {\intbobb}{\int_{\bar{\bar{\Omega}}_{20}}}
\newcommand {\intib}{\int_{\bar{\Omega}_i}}
\newcommand {\intjb}{\int_{\bar{\Omega}_j}}
\newcommand {\intkb}{\int_{\bar\Omega_k}}
\newcommand {\intlb}{\int_{\bar\Omega_\ell}}
\newcommand {\intie}{\int_{\Omega_i^e}}
\newcommand {\intje}{\int_{\Omega_j^e}}
\newcommand {\intpa}{\int_{\partial\bar{\Omega}_1}}
\newcommand {\intpb}{\int_{\partial\bar{\Omega}_2}}
%\newcommand {\intpi}{\int_{\partial{\Omega}_i^e}}
%\newcommand {\intpj}{\int_{\partial{\Omega}_j^e}}
%\newcommand {\intpk}{\int_{\partial{\Omega}_k^e}}
\newcommand {\intpi}{\int_{\Gamma_i^e}}
\newcommand {\intpj}{\int_{\Gamma_j^e}}
\newcommand {\intpk}{\int_{\Gamma_k^e}}
\newcommand {\intpio}{\int_{\Gamma_{i0}^{e}}}
\newcommand {\intpjo}{\int_{\Gamma_{j0}^{e}}}
\newcommand {\intpko}{\int_{\Gamma_{k0}^{e}}}

% Indices
\newcommand {\mra}{\mathrm{a}}
\newcommand {\mrb}{\mathrm{b}}
\newcommand {\mrc}{\mathrm{c}}
\newcommand {\mrd}{\mathrm{d}}
\newcommand {\mre}{\mathrm{e}}
\newcommand {\mrf}{\mathrm{f}}
\newcommand {\mrg}{\mathrm{g}}
\newcommand {\mrh}{\mathrm{h}}
\newcommand {\mri}{\mathrm{i}}
\newcommand {\mrj}{\mathrm{j}}
\newcommand {\mrk}{\mathrm{k}}
\newcommand {\mrl}{\mathrm{l}}
\newcommand {\mrm}{\mathrm{m}}
\newcommand {\mrn}{\mathrm{n}}
\newcommand {\mro}{\mathrm{o}}
\newcommand {\mrp}{\mathrm{p}}
\newcommand {\mrq}{\mathrm{q}}
\newcommand {\mrr}{\mathrm{r}}
\newcommand {\mrs}{\mathrm{s}}
\newcommand {\mrt}{\mathrm{t}}
\newcommand {\mru}{\mathrm{u}}
\newcommand {\mrv}{\mathrm{v}}
\newcommand {\mrw}{\mathrm{w}}
\newcommand {\mrx}{\mathrm{x}}
\newcommand {\mry}{\mathrm{y}}
\newcommand {\mrz}{\mathrm{z}}
\newcommand {\mrP}{\mathrm{P}}
\newcommand {\mrX}{\mathrm{X}}

% Vectors (Bold lower case)
\newcommand {\ma}{\mathbf{a}}
%\newcommand {\mb}{\mathbf{b}}
\newcommand {\mcc}{\mathbf{c}}
\newcommand {\md}{\mathbf{d}}
\newcommand {\me}{\mathbf{e}}
\newcommand {\mf}{\mathbf{f}}
\newcommand {\mg}{\mathbf{g}}
\newcommand {\mh}{\mathbf{h}}
\newcommand {\mii}{\mathbf{i}}
\newcommand {\mj}{\mathbf{j}}
\newcommand {\mk}{\mathbf{k}}
\newcommand {\ml}{\mathbf{l}}
\newcommand {\mm}{\mathbf{m}}
\newcommand {\mn}{\mathbf{n}}
\newcommand {\mo}{\mathbf{o}}
\newcommand {\mpp}{\mathbf{p}}
\newcommand {\mq}{\mathbf{q}}
\newcommand {\mr}{\mathbf{r}}
%\newcommand {\ms}{\mathbf{s}}
\newcommand {\mt}{\mathbf{t}}
\newcommand {\muu}{\mathbf{u}}
\newcommand {\mv}{\mathbf{v}}
\newcommand {\mw}{\mathbf{w}}
\newcommand {\mx}{\mathbf{x}}
\newcommand {\my}{\mathbf{y}}
\newcommand {\mz}{\mathbf{z}}

\newcommand {\ba}{\boldsymbol{a}}
\newcommand {\bb}{\boldsymbol{b}}
\newcommand {\bbbar}{\boldsymbol{\bar{b}}}
\newcommand {\bkbar}{\boldsymbol{\bar{k}}}
\newcommand {\bbhat}{\boldsymbol{\hat{b}}}
\newcommand {\bkhat}{\boldsymbol{\hat{k}}}

\newcommand {\bKbar}{\boldsymbol{\bar{K}}}


\newcommand {\bc}{\boldsymbol{c}}
\newcommand {\bcbar}{\boldsymbol{\bar{c}}}


\newcommand {\bd}{\boldsymbol{d}}
\newcommand {\be}{\boldsymbol{e}}
\newcommand {\bff}{\boldsymbol{f}}
\newcommand {\bg}{\boldsymbol{g}}
\newcommand {\bh}{\boldsymbol{h}}
\newcommand {\bi}{\boldsymbol{i}}
\newcommand {\bj}{\boldsymbol{j}}
\newcommand {\bk}{\boldsymbol{k}}
\newcommand {\bl}{\boldsymbol{l}}
\newcommand {\blhat}{\boldsymbol{\hat{l}}}
\newcommand {\bell}{\boldsymbol{\ell}}
\newcommand {\bellhat}{\boldsymbol{\hat{\ell}}}

\newcommand {\bm}{\boldsymbol{m}}
\newcommand {\bmbar}{\boldsymbol{\bar{m}}}
\newcommand {\bmhat}{\boldsymbol{\hat{m}}}
\newcommand {\bmchk}{\boldsymbol{\check{m}}}

\newcommand {\bn}{\boldsymbol{n}}
\newcommand {\bnbar}{\boldsymbol{\bar{n}}}
\newcommand {\babar}{\boldsymbol{\bar{a}}}

\newcommand {\dotbnbar}{\boldsymbol{\dot{{\bar{{n}}}}}}

\newcommand {\nbar}{\bar{n}}

\newcommand {\bo}{\boldsymbol{o}}
\newcommand {\bp}{\boldsymbol{p}}
\newcommand {\bq}{\boldsymbol{q}}
\newcommand {\br}{\boldsymbol{r}}
\newcommand {\bs}{\boldsymbol{s}}
\newcommand {\bt}{\boldsymbol{t}}
\newcommand {\bu}{\boldsymbol{u}}
\newcommand {\bv}{\boldsymbol{v}}
\newcommand {\bw}{\boldsymbol{w}}
\newcommand {\bx}{\boldsymbol{x}}
\newcommand {\by}{\boldsymbol{y}}
\newcommand {\bz}{\boldsymbol{z}}
%\newcommand {\bf0}{\boldsymbol{0}}
%\newcommand {\bnu}{\boldsymbol{\nu}}
\newcommand {\bmu}{\boldsymbol{\mu}}

\newcommand {\bmubar}{\boldsymbol{\bar{\mu}}}
\newcommand {\bmuhat}{\boldsymbol{\hat{\mu}}}
\newcommand {\bmuchk}{\boldsymbol{\check{\mu}}}
% Greek
\newcommand {\balp}{\mbox{\boldmath$\alpha$}}
\newcommand {\bbet}{\mbox{\boldmath$\beta$}}
\newcommand {\bdel}{\mbox{\boldmath$\delta$}}
\newcommand {\blam}{\mbox{\boldmath$\lambda$}}
\newcommand {\bnu}{\mbox{\boldmath$\nu$}}
\newcommand {\bphi}{\mbox{\boldmath$\phi$}}
\newcommand {\bpsi}{\mbox{\boldmath$\psi$}}
\newcommand {\bvphi}{\mbox{\boldmath$\varphi$}}
\newcommand {\brho}{\mbox{\boldmath$\rho$}}
\newcommand {\bxi}{\mbox{\boldmath$\xi$}}
\newcommand {\bet}{\mbox{\boldmath$\eta$}}
\newcommand {\btheta}{\mbox{\boldmath$\theta$}}
\newcommand {\bome}{\mbox{\boldmath$\omega$}}

% 2nd Order Tensors (Bold upper case)
\newcommand {\mA}{\mathbf{A}}
\newcommand {\mB}{\mathbf{B}}
\newcommand {\mC}{\mathbf{C}}
\newcommand {\mD}{\mathbf{D}}
\newcommand {\mE}{\mathbf{E}}
\newcommand {\mF}{\mathbf{F}}
\newcommand {\mG}{\mathbf{G}}
\newcommand {\mH}{\mathbf{H}}
\newcommand {\mI}{\mathbf{I}}
\newcommand {\mJ}{\mathbf{J}}
\newcommand {\mK}{\mathbf{K}}
\newcommand {\mL}{\mathbf{L}}
\newcommand {\mM}{\mathbf{M}}
\newcommand {\mN}{\mathbf{N}}
\newcommand {\mO}{\mathbf{O}}
\newcommand {\mP}{\mathbf{P}}
\newcommand {\mQ}{\mathbf{Q}}
\newcommand {\mR}{\mathbf{R}}
\newcommand {\mS}{\mathbf{S}}
\newcommand {\mT}{\mathbf{T}}
\newcommand {\mU}{\mathbf{U}}
\newcommand {\mV}{\mathbf{V}}
\newcommand {\mW}{\mathbf{W}}
\newcommand {\mX}{\mathbf{X}}
\newcommand {\mY}{\mathbf{Y}}
\newcommand {\mZ}{\mathbf{Z}}

\newcommand {\bA}{\boldsymbol{A}}
\newcommand {\bB}{\boldsymbol{B}}
\newcommand {\bC}{\boldsymbol{C}}
\newcommand {\bD}{\boldsymbol{D}}
\newcommand {\bE}{\boldsymbol{E}}
\newcommand {\bF}{\boldsymbol{F}}
\newcommand {\bG}{\boldsymbol{G}}
\newcommand {\bH}{\boldsymbol{H}}
\newcommand {\bI}{\boldsymbol{I}}
\newcommand {\bJ}{\boldsymbol{J}}
\newcommand {\bK}{\boldsymbol{K}}
\newcommand {\bL}{\boldsymbol{L}}

\newcommand {\bM}{\boldsymbol{M}}

\newcommand {\bMbar}{\boldsymbol{\bar{M}}}
\newcommand {\bMhat}{\boldsymbol{\hat{M}}}
\newcommand {\bMchk}{\boldsymbol{\check{M}}}

\newcommand {\bGamma}{\boldsymbol{\Gamma}}
\newcommand {\bOmega}{\boldsymbol{\Omega}}
\newcommand {\bOmegabar}{\boldsymbol{\bar\Omega}}

\newcommand {\bGammabar}{\boldsymbol{\bar{\Gamma}}}
\newcommand {\bGammahat}{\boldsymbol{\hat{\Gamma}}}

\newcommand {\bN}{\boldsymbol{N}}
\newcommand {\bO}{\boldsymbol{O}}
\newcommand {\bP}{\boldsymbol{P}}
\newcommand {\bQ}{\boldsymbol{Q}}
\newcommand {\bR}{\boldsymbol{R}}
\newcommand {\bS}{\boldsymbol{S}}
\newcommand {\bT}{\boldsymbol{T}}
\newcommand {\bU}{\boldsymbol{U}}
\newcommand {\bV}{\boldsymbol{V}}
\newcommand {\bW}{\boldsymbol{W}}
\newcommand {\bX}{\boldsymbol{X}}
\newcommand {\bY}{\boldsymbol{Y}}
\newcommand {\bZ}{\boldsymbol{Z}}

\newcommand {\eps}{\varepsilon}
\newcommand {\sig}{\sigma}
\newcommand {\vphi}{\varphi}
\newcommand {\beps}{\mbox{\boldmath$\varepsilon$}}
\newcommand {\bLam}{\mbox{\boldmath$\Lambda$}}

\newcommand {\bsig}{\mbox{\boldmath$\sigma$}}
\newcommand {\bsigbar}{\mbox{\boldmath$\bar{\sigma}$}}

\newcommand {\bVc}{\boldsymbol{V}_{\!\!\!\mrc}}
\newcommand {\bVn}{\boldsymbol{V}_{\!\!\mrn}}
\newcommand {\bVell}{\boldsymbol{V}_{\!\!\!\mathrm{\ell}}}

\newcommand {\bSig}{\mbox{\boldmath$\Sigma$}}
\newcommand {\btau}{\mbox{\boldmath$\tau$}}
\newcommand {\bbphi}{\mbox{\boldmath$\Phi$}}
\newcommand {\bom}{\mbox{\boldmath$\omega$}}
\newcommand {\bOme}{\mbox{\boldmath$\Omega$}}
\newcommand {\bThe}{\mbox{\boldmath$\Theta$}}
\newcommand {\bXi}{\mbox{\boldmath$\Xi$}}
\newcommand {\kd}[1]{\delta_{#1}}
\newcommand {\bone}{\mathbf{1}}
\newcommand {\bxih}{\bxi_\mathrm{h}}
\newcommand {\Boxh}{\Box_\mathrm{h}}

% 4th Order Tensors
\newcommand {\bbA}{\mathbb{A}}
\newcommand {\bbB}{\mathbb{B}}
\newcommand {\bbC}{\mathbb{C}}
\newcommand {\bbD}{\mathbb{D}}
\newcommand {\bbE}{\mathbb{E}}
\newcommand {\bbF}{\mathbb{F}}
\newcommand {\bbG}{\mathbb{G}}
\newcommand {\bbH}{\mathbb{H}}
\newcommand {\bbI}{\mathbb{I}}
\newcommand {\bbJ}{\mathbb{J}}
\newcommand {\bbK}{\mathbb{K}}
\newcommand {\bbL}{\mathbb{L}}
\newcommand {\bbM}{\mathbb{M}}
\newcommand {\bbN}{\mathbb{N}}
\newcommand {\bbO}{\mathbb{O}}
\newcommand {\bbP}{\mathbb{P}}
\newcommand {\bbQ}{\mathbb{Q}}
\newcommand {\bbR}{\mathbb{R}}
\newcommand {\bbS}{\mathbb{S}}
\newcommand {\bbT}{\mathbb{T}}
\newcommand {\bbU}{\mathbb{U}}
\newcommand {\bbV}{\mathbb{V}}
\newcommand {\bbW}{\mathbb{W}}
\newcommand {\bbX}{\mathbb{X}}
\newcommand {\bbY}{\mathbb{Y}}
\newcommand {\bbZ}{\mathbb{Z}}

\newcommand {\IR}{{\rm\kern.24em
   \vrule width.02em height1.53ex depth-.05ex
   \kern-.3em R}}
\newcommand {\ic}{{\rm\kern.20em
   \vrule width.02em height1.0ex depth-.05ex
   \kern-.22em c}}
%\newcommand {\ia}{{\rm\kern.20em
%   \vrule width.02em height1.2ex depth-.05ex
%   \kern-.32em \textit{a}}}
\newcommand {\ia}{{\rm\kern.20em
   \vrule width.02em height1.05ex depth-.0ex
   \kern-.25em a}}
\newcommand {\IC}{{\rm\kern.24em
   \vrule width.02em height1.4ex depth-.05ex
   \kern-.26em C}}
\newcommand {\ID}{{\rm\kern.34em
   \vrule width.02em height1.5ex depth-.05ex
   \kern-.36em D}}
%\newcommand {\IIo}{{\rm\kern.30em
%   \vrule width.02em height1.55ex depth-.05ex
%   \kern-.32em I}}
%\newcommand {\II}{{\rm\kern.30em
%   \vrule width.02em height1.55ex depth-.05ex
%   \kern-.32em I}_{ijkl}}
%\newcommand {\IIs}{{\rm\kern.30em
%   \vrule width.02em height1.55ex depth-.05ex
%   \kern-.32em I}^{s}_{ijkl}}
\newcommand {\IS}{{\rm\kern.24em
   \vrule width.02em height1.6ex depth.05ex
   \kern-.26em S}}
\newcommand {\IT}{{\rm\kern.50em
   \vrule width.02em height1.55ex depth-.05ex
   \kern-.52em T}}
\newcommand {\Sa}{\ds\frac{1}{2(1-\nu)}}
\newcommand {\Sb}{\ds\frac{3-4\nu}{4(1-\nu)}}
\newcommand {\Sc}{\ds\frac{1}{4(1-\nu)(3-4\nu)}}
\newcommand {\SC}{\ds\frac{1}{2(1-\nu)(3-4\nu)}}
\newcommand {\Sco}{\ds\frac{1}{4(1-\nu)(3-4\nu)R^2_0}}
\newcommand {\IE}{{\rm\kern.24em
   \vrule width.02em height1.55ex depth-.05ex
   \kern-.33em E}}
\newcommand {\IEa}{{\rm\kern.24em
   \vrule width.02em height1.55ex depth-.05ex
   \kern-.33em E}^{1}_{ijkl}}
\newcommand {\IEb}{{\rm\kern.24em
   \vrule width.02em height1.55ex depth-.05ex
   \kern-.33em E}^{2}_{ijkl}}

% Spaces
\newcommand {\sA}{\mathcal{A}}

\newcommand {\sB}{\mathcal{B}}
\newcommand {\sC}{\mathcal{C}}


\newcommand {\bkB}{\boldsymbol{\mathfrak{b}}}
\newcommand {\bkL}{\boldsymbol{\mathfrak{l}}}
\newcommand {\bkC}{\boldsymbol{\mathfrak{c}}}

\newcommand {\bsB}{\boldsymbol{\mathcal{B}}}
\newcommand {\bsL}{\boldsymbol{\mathcal{L}}}
\newcommand {\bsC}{\boldsymbol{\mathcal{C}}}

\newcommand {\sD}{\mathcal{D}}
\newcommand {\sE}{\mathcal{E}}
\newcommand {\sF}{\mathcal{F}}
\newcommand {\sG}{\mathcal{G}}
\newcommand {\sH}{\mathcal{H}}
\newcommand {\sI}{\mathcal{I}}
\newcommand {\sJ}{\mathcal{J}}
\newcommand {\sK}{\mathcal{K}}
\newcommand {\sL}{\mathcal{L}}
\newcommand {\sM}{\mathcal{M}}
\newcommand {\sN}{\mathcal{N}}
\newcommand {\sO}{\mathcal{O}}
\newcommand {\sP}{\mathcal{P}}
\newcommand {\sQ}{\mathcal{Q}}
\newcommand {\sR}{\mathcal{R}}
\newcommand {\sS}{\mathcal{S}}
\newcommand {\sT}{\mathcal{T}}
\newcommand {\sU}{\mathcal{U}}
\newcommand {\sV}{\mathcal{V}}
\newcommand {\sW}{\mathcal{W}}
\newcommand {\sX}{\mathcal{X}}
\newcommand {\sY}{\mathcal{Y}}
\newcommand {\sZ}{\mathcal{Z}}

\newcommand {\bsM}{\boldsymbol{\mathcal{M}}}
%vector a:
\newcommand {\vaua}{\ba_\alpha}
\newcommand {\vaa}{\ba^\alpha}

\newcommand {\vaub}{\ba_\beta}
\newcommand {\vab}{\ba^\beta}

\newcommand {\vaug}{\ba_\gamma}
\newcommand {\vag}{\ba^\gamma}

\newcommand {\vaud}{\ba_\delta}
\newcommand {\vad}{\ba^\delta}

\newcommand {\vauacb}{\ba_{\alpha,\beta}}
\newcommand {\vaugcd}{\ba_{\gamma,\delta}}

\newcommand {\vtiln}{\tilde{\bn}}
\newcommand {\vtilNcb}{\tilde{\bN}_{,\beta}}
\newcommand {\vtilNca}{\tilde{\bN}_{,\alpha}}

\newcommand {\vNcb}{\bN_{,\beta}}
\newcommand {\vNca}{\bN_{,\alpha}}
\newcommand {\vNcg}{\bN_{,\gamma}}
\newcommand {\vNcd}{\bN_{,\delta}}

\newcommand {\vNcab}{\bN_{,\alpha\beta}}
\newcommand {\vNcgd}{\bN_{,\gamma\delta}}

% Finite Elements
\newcommand{\Pint}[1]{\Pi_{\mathrm{int}#1}}
\newcommand{\Pext}[1]{\Pi_{\mathrm{ext}#1}}
\newcommand{\Pic}{\Pi_{\mathrm{c}}}
\newcommand{\fint}[1]{\mf_{\mathrm{int}#1}}
\newcommand{\fext}[1]{\mf_{\mathrm{ext}#1}}
\newcommand{\fc}[1]{\mf_{\mathrm{c}#1}}
\newcommand{\kint}[1]{\mk_{\mathrm{int}#1}}
\newcommand{\kc}[1]{\mk_{\mathrm{c}#1}}

% Coarse-Graining
%\newcommand{\mhx}{{\bf\hat\mx}}
%\newcommand{\bhx}{{\bf\hat\bx}}
%\newcommand{\mhX}{{\bf\hat\mX}}
\newcommand{\mhx}{{\mz}}
\newcommand{\mhX}{{\mZ}}

% Variations
\newcommand {\dphi}{\delta\bvphi}

% Operators
\newcommand {\Ass}[2]{\kern 0.9ex \vrule width0.45em height0.2ex depth0ex \kern -2.1ex \bigwedge_{#1}^{#2}}
\newcommand {\ASS}[2]{\kern 1.45ex \vrule width0.5em height0.2ex depth0ex \kern -2.65ex \bigwedge_{#1}^{#2}}

%tensors
\newcommand {\Cabgd}{{c}^{\alpha\beta\gamma\delta}}
\newcommand {\Dabgd}{{d}^{\alpha\beta\gamma\delta}}
\newcommand {\Eabgd}{{e}^{\alpha\beta\gamma\delta}}
\newcommand {\Fabgd}{{f}^{\alpha\beta\gamma\delta}}
\newcommand {\tCabgd}{\tilde{c}^{\alpha\beta\gamma\delta}}
\newcommand {\tDabgd}{\tilde{d}^{\alpha\beta\gamma\delta}}
\newcommand {\tEabgd}{\tilde{e}^{\alpha\beta\gamma\delta}}
\newcommand {\tFabgd}{\tilde{f}^{\alpha\beta\gamma\delta}}

\newcommand {\Babgd}{k^{\alpha\beta\gamma\delta}}
\newcommand {\babgd}{b^{\alpha\beta\gamma\delta}}

\newcommand {\cabgd}{{c}^{\alpha\beta\gamma\delta}}
\newcommand {\dabgd}{{d}^{\alpha\beta\gamma\delta}}
\newcommand {\eabgd}{{e}^{\alpha\beta\gamma\delta}}
\newcommand {\fabgd}{{f}^{\alpha\beta\gamma\delta}}


\newcommand {\mabgd}{m^{\alpha\beta\gamma\delta}}
\newcommand {\mgate}{m^{\gamma\alpha\theta\epsilon}}
\newcommand {\mdbte}{m^{\delta\beta\theta\epsilon}}
\newcommand {\mtagd}{m^{\theta\alpha\gamma\delta}}
\newcommand {\mebgd}{m^{\epsilon\beta\gamma\delta}}


% Colors
%\definecolor{col}{rgb}{0.6,0.1,0.5}

% Packed itemize
\newenvironment{packeditemize}{
\begin{itemize}
  %\setlength{\itemindent}{-10pt}
  \setlength{\listparindent}{-10pt}
  \setlength{\itemsep}{2pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}} 

